A Factor-Graph Approach to Algebraic Topology, With Applications to Kramers--Wannier Duality

Algebraic topology studies topological spaces with the help of tools from abstract algebra. The main focus of this paper is to show that many concepts from algebraic topology can be conveniently expressed in terms of (normal) factor graphs. As an application, we give an alternative proof of a classical duality result of Kramers and Wannier, which expresses the partition function of the two-dimensional Ising model at a low temperature in terms of the partition function of the two-dimensional Ising model at a high temperature. Moreover, we discuss analogous results for the three-dimensional Ising model and the Potts model.

==> figtex/eg1.tex <==
\begin{tikzpicture}
	\node at (0,0){\input{figtex/eg1p}};
	\def\clr{red}
	\node at (0,0){\input{figtex/eg1d}};
\end{tikzpicture}


==> figtex/eg1d.tex <==
\begin{tikzpicture}[scale=2, >=latex,
	every loop/.style={in=60,out=120,looseness=10},
	every node/.style={draw, circle, fill, minimum size=1.5mm, inner sep=0mm, \clr}]
	\node(v1)[label={left:{$S_1$}}] at (0,0){};
	\draw[\clr]
	(v1) edge[->, loop above] (a)
		;
\end{tikzpicture}


==> figtex/eg1p.tex <==
\begin{tikzpicture}[scale=2, >=latex,
	every node/.style={draw, circle, fill, minimum size=1.5mm, inner sep=0mm, \clr}]
	\node(v1)[label={left:{$v_1$}}] at (0,0){};
	\node(v2)[label={right:{$v_2$}}] at (1,0){};
	\draw[\clr]
	(v1) edge[->] (v2)
		;
\end{tikzpicture}


==> figtex/eg2.tex <==
\begin{tikzpicture}
	\node at (0,0){\input{figtex/eg2p}};
	\def\clr{red}
	\node at (1.75,0){\input{figtex/eg2d}};
\end{tikzpicture}


==> figtex/new-figs/preamble.tex <==
%\documentclass[10pt]{article} \usepackage{fullpage}

%\usepackage{balance}
%\usepackage{flushend}
\usepackage[export]{adjustbox}


\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{thmtools}
\renewcommand\thmcontinues[2]{#2Continued}

\usepackage{tikz}
\usetikzlibrary{calc, arrows, decorations.markings, shapes, positioning, 3d}
\usetikzlibrary{matrix}
\usepackage{xifthen}
% calc for node between two nodes
% decoration for ciliation

\usepackage{calc} % Included for the clockwise arrow
\usepackage{subfigure}
%\usepackage{caption}
\usepackage{graphicx}
\usepackage{comment}
\usepackage{color}

%\usepackage{enumitem}
%\setlist{noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt}

\usepackage{timestamp}
\date{}
%\pagenumbering{arabic}
%\usepackage{nopageno}


\newcommand{\F}{\mathbb F}
\newcommand{\R}{\mathbb R}
\newcommand{\img}{ {\rm im\,}}
\newcommand{\In}{ {\rm In\,}}
\newcommand{\Out}{ {\rm Out\,}}
%\newcommand{\ker}{ {\rm Ker}}
\newcommand{\A}{{\cal A}}
\newcommand{\G}{{\cal G}}
\renewcommand{\H}{{\cal H}}
\newcommand{\V}{{\cal V}}
\newcommand{\E}{{\cal E}}
\newcommand{\X}{{\cal X}}
\newcommand{\Y}{{\cal Y}}
\newcommand{\D}{{\cal D}}
\newcommand{\T}{{\cal T}}
\newcommand{\s}{{\cal S}}
\newcommand{\vnfg}{{\cal F}}
\newcommand{\B}{{\cal B}}
\newcommand{\code}{{\cal C}}
\newcommand{\I}{{\cal I}}
\newcommand{\eqpunc}{\,}
\newcommand{\dg}{\mathrm{d}}

\newcommand{\ft}{Fourier-transformed }

\newcommand*{\qedb}{\hfill\ensuremath{\blacksquare}}%
\newcommand*{\qedw}{\hfill\ensuremath{\square}}%


\newtheorem{theorem}{Theorem}
\newtheorem{example}[theorem]{Example}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{lemma}[theorem]{Lemma}


\newcommand{\refrecipe}{Construction}
\newtheorem{recipe}[theorem]{\refrecipe}
\newcommand{\exterior}{partition }
%\renewcommand{\exterior}{exterior }


\specialcomment{comment}{\begingroup\color{blue}}{\endgroup}
\specialcomment{commentold}{\begingroup\color{blue}}{\endgroup}
%\specialcomment{note}{\color{blue}}{\color{black}}

\newcommand{\selfnote}[1]{\textbf{\color{blue}{selfnote: #1}}}


%\renewcommand\thefootnote{\textcolor{red}{\arabic{footnote}}}


%\documentclass[10pt]{article} \usepackage{fullpage}

%\widowpenalties 1 10000
%\raggedbottom






%% Arrow for conditional and constrained nodes
%\tikzset{->-out/.style={decoration={
%  markings,
%  mark=at position #1 with {\arrow{triangle 45}}},postaction={decorate}}}
%\tikzset{->-in/.style={decoration={
%  markings,
%  mark=at position #1 with {\arrowreversed{triangle 45}}},postaction={decorate}}}

%%% Ciliation
%% change value of \pgftransformscale to change ciliation size
%\tikzset{ --o/.style={
%  decoration={ markings,
%  mark=at position .95 with {\pgftransformscale{.8}\arrowreversed[line width=0mm]{*}}},
%  postaction={decorate}
%  }
%}
%
%
%
%\tikzset{-o-/.style={
%  decoration={ markings,
%  mark=at position .66 with {\pgftransformscale{.8}\arrowreversed[line width=0mm]{*}}},
%  postaction={decorate}
%  }
%}
%
%\tikzset{o--/.style={
%  decoration={ markings,
%  mark=at position 0 with {\pgftransformscale{.8}\arrowreversed[line width=0mm]{*}}},
%  postaction={decorate}
%  }
%}

%\tikzstyle dongle=[circle,draw=none,fill=black,inner sep=0pt, minimum size=#1]
%\tikzstyle ciliatednode=[vertex,pin={[pin distance=1mm,pin edge={semitransparent,red},ciliation]#1:{}}]


%% Close the box
%\newcommand{\clbox}[4]{+(#1,#2) rectangle +(#3,#4);}



==> figtex/new-figs/tikz-preamble.tex <==
\input{cube} % \angle is defined here
\def\extend{.4}
\def\extendclr{gray!50}
\def\extendclr{red!50}
\def\extendtype{dashed}
\input{cube-orient-ext}
%\input{cube-orient}
%\input{cubenfg3}

%\input{cubenfgbd3ext}
\input{cubenfgbd3}
\input{cubenfgbd2}
%\input{cubenfgbd1ext}
\input{cubenfgbd1}
%\input{cubenfgbd2_2}
%\input{cubenfg}
\input{cubedang}

\input{vstyles-common}



\def\clr{}
\def\linetype{}
\def\subscale{1}	
\def\dist{1}	
\tikzset{vcaption/.style={node distance=.0cm, font=\scriptsize} }



% Face orientation 


%\begin{tikzpicture}
%\begin{scope}[canvas is xy plane at z=2]
%%\draw (0,0) circle (1cm);
%%\draw (-1,0) -- (1,0) (0,-1) -- (0,1);
%%\counterclockwise{$S_3$}
%\draw (0,1.0) arc (85:-240:1.0);%
%\end{scope}
%\end{tikzpicture}

\makeatletter
\newlength\@SizeOfCirc%
\newcommand{\CricArrowRight}[1]{%
	\setlength{\@SizeOfCirc}{\maxof{\widthof{#1}}{\heightof{#1}}}%
	\tikz [>=angle 90, x=1.0ex,y=1.0ex,line width=.1ex, draw=black]%
	\draw [->,anchor=center]%
		node[fill=none, draw=none] (0,0) {#1}%
		(0,1.0\@SizeOfCirc) arc (85:-240:1.0\@SizeOfCirc);%
}%
\newcommand{\clockwise}[1]{%
	\setlength{\@SizeOfCirc}{\maxof{\widthof{#1}}{\heightof{#1}}}%
	\tikz [>=angle 90, x=1.0ex,y=1.0ex,line width=.1ex, draw=black]%
	\draw [->,anchor=center]%
		node[fill=none, draw=none] (0,0) {#1}%
		(0,1.0\@SizeOfCirc) arc (85:-240:1.0\@SizeOfCirc);%
}%
\newcommand{\counterclockwise}[1]{%
	\setlength{\@SizeOfCirc}{\maxof{\widthof{#1}}{\heightof{#1}}}%
	\begin{tikzpicture}[>=angle 90, x=1.0ex,y=1.0ex,line width=.1ex, draw=black]%
	\draw [->,anchor=center]%
		node[fill=none, draw=none] (0,0) {#1}%
		(0,1.0\@SizeOfCirc) arc (-275:40:1.0\@SizeOfCirc);%
	\end{tikzpicture}
}%
%
\makeatother


\def\clocksize{4}
\def\angstart{0}
\def\angend{45}
\newcommand{\clockxy}[1]{%
	\tikz[>=angle 90, x=1.0ex,y=1.0ex,line width=.1ex, draw=black]%
	\draw [->,anchor=center]%
		node[fill=none, draw=none] (0,0) {#1}%
		(0,{1*\clocksize}) arc (0:\angend-360:{.75*\clocksize});%
}%
\newcommand{\clockxz}[1]{%
	\tikz[>=angle 90, x=1.0ex,y=1.0ex,line width=.1ex, draw=black]%
	\draw [->,anchor=center]%
		node[fill=none, draw=none] (0,0) {#1}%
		(0,{.5*\clocksize}) arc (0:\angend-360:{\clocksize*\cosine} and {\clocksize*\sine});%
}%
\newcommand{\clockyz}[1]{%
	\tikz[>=angle 90, x=1.0ex,y=1.0ex,line width=.1ex, draw=black]%
	\draw [->,anchor=center]%
		node[fill=none, draw=none] (0,0) {#1}%
		(0,{.5*\clocksize}) arc (0:\angend-360:{\clocksize*\cosine} and {\clocksize*\sine});%
}%
%
\newcommand{\counterclockxy}[1]{%
	\tikz[>=angle 90, x=1.0ex,y=1.0ex,line width=.1ex, draw=black]%
	\draw [->,anchor=center]%
		node[fill=none, draw=none] (0,0) {#1}%
		(0,{1*\clocksize}) arc (0:\angend-360:{.75*\clocksize});%
}%
\newcommand{\counterclockxz}[1]{%
	\tikz[>=angle 90, x=1.0ex,y=1.0ex,line width=.1ex, draw=black]%
	\draw [->,anchor=center]%
		node[fill=none, draw=none] (0,0) {#1}%
		(0,{.5*\clocksize}) arc (-275:40:{\clocksize*\cosine} and {\clocksize*\sine});%
}%
\newcommand{\counterclockyz}[1]{%
	\tikz[>=angle 90, x=1.0ex,y=1.0ex,line width=.1ex, draw=black]%
	\draw [->,anchor=center]%
		node[fill=none, draw=none] (0,0) {#1}%
		(0,{.5*\clocksize}) arc (-270:40:{\clocksize*\cosine} and {\clocksize*\sine});%
}%
%


%\newcommand{\clockxz}[1]{%
%	\settowidth{\SizeofCirc}{\pgfinterruptpicture A \endpgfinterruppicture}%
%	\begin{tikzpicture}[>=angle 90, x=1.0ex,y=1.0ex,line width=.1ex, draw=black]%
%%\begin{scope}[canvas is xz plane at y=0]
%	\draw [->,anchor=center]%
%		node[fill=none, draw=none] (0,0) {#1}%
%		%(0,1.0\@SizeOfCirc) arc (85:-240:1\@SizeOfCirc);%
%		(0,1.0\SizeofCirc) arc (85:-240:1.0\SizeofCirc);%
%%\end{scope}
%	\end{tikzpicture}
%}%

% Ciliation take 2
\tikzstyle ciliation=[circle,draw,fill=white,inner sep=0pt, minimum size=#1]
\tikzset{ ciliatednode/.style 2 args
	={ pin={[pin distance=0mm, ciliation=#2]#1:{}} }
	%={pin={} }
}
% gray ciliation
\tikzstyle gciliation=[gray, circle,draw,fill=white,inner sep=0pt, minimum size=#1]
\tikzset{ gciliatednode/.style 2 args
	={ pin={[pin distance=0mm, gciliation=#2]#1:{}} }
	%={pin={} }
}
% extend ciliation
\tikzstyle extendciliation=[\extendclr, circle,draw,fill=white,inner sep=0pt, minimum size=#1]
\tikzset{ extendciliatednode/.style 2 args
	={ pin={[pin distance=0mm, extendciliation=#2]#1:{}} }
	%={pin={} }
}

% dongle
\tikzset{ --|/.style={
  decoration={ markings,
  mark=at position 1 with {\pgftransformscale{1.5}\arrowreversed[line width=0mm]{|}}},
  postaction={decorate}
  }
}


%%\newcommand\cube{
%\newcommand\cube[3]{
%%\fill[fill=red!40, draw=black,shift={(0:#1)},shift={(90:#2)}, shift={(45:#3)}]
%% define the points  
%	\def\angle{30}
%	\pgfmathsetmacro\cos{cos(\angle)}
%	\pgfmathsetmacro\sin{sin(\angle)}
%	\path[shift={(0:#1)},shift={(90:#2)}, shift={(\angle:#3*\cos)}]
%		%(0,0)     coordinate (A)  (1,0)     coordinate (B) % bottom
%		%(1.5,0.5) coordinate (C)  (0.5,0.5) coordinate (D)
%		%(0,1)     coordinate (E)  (1,1)     coordinate (F) % top  add 1 for y
%		%(1.5,1.5) coordinate (G)  (0.5,1.5) coordinate (H);
%		(0,0)  coordinate (A)  (1,0)     coordinate (B) % bottom
%		+(\angle:\cos) coordinate (C)  (\angle:\cos) coordinate (D)
%		(0,1)  coordinate (E) +(\angle:\cos) coordinate (H)   % top  add 1 for y
%		(1,1)  coordinate (F) +(\angle:\cos) coordinate (G)  ;
%%        ($(A)!0.5!(C)$) coordinate (O)   % middle of A--C
%%        ($(E)!0.5!(G)$) coordinate (P);%   
%	\draw[draw=black]
%		(A) -- (E) (B) -- (F) (C) -- (G)  % lateral 
%		(A) -- (B) -- (C) % bottom 
%		(E) -- (F) -- (G) -- (H) -- (E); % top
%	% dashed is an option
%	\draw[fill=red!40, draw=black]
%		(D) -- (H) (D) -- (C) (D) -- (A);  
%% shading
%	%\node[fill=white,opacity=.8, minimum height=1.47cm, minimum width=1.47cm] at ($(A)+(.5,.5)$) {};
%		\def\gap{.99}
%		% front
%		\node[inner sep=0,minimum size=0](cf) at (barycentric cs:A=1,B=1,F=1,E=1){};
%		\path(cf) -- coordinate[pos=\gap] (Af) (A.0);
%		\path(cf) -- coordinate[pos=\gap] (Bf) (B);
%		\path(cf) -- coordinate[pos=\gap] (Ff) (F);
%		\path(cf) -- coordinate[pos=\gap] (Ef) (E);
%		\draw(F)--(Ff);
%		% right
%		\node[inner sep=0,minimum size=0](cr) at (barycentric cs:B=1,C=1,G=1,F=1){};
%		\path(cr) -- coordinate[pos=\gap] (Br) (B);
%		\path(cr) -- coordinate[pos=\gap] (Cr) (C);
%		\path(cr) -- coordinate[pos=\gap] (Gr) (G);
%		\path(cr) -- coordinate[pos=\gap] (Fr) (F);
%		% top
%		\node[inner sep=0,minimum size=0](ct) at (barycentric cs:E=1,F=1,G=1,H=1){};
%		\path(ct) -- coordinate[pos=\gap] (Et) (E);
%		\path(ct) -- coordinate[pos=\gap] (Gt) (G);
%		\path(ct) -- coordinate[pos=\gap] (Ft) (F);
%		\path(ct) -- coordinate[pos=\gap] (Ht) (H);
%
%	\path[fill=white,fill opacity=.6]
%		(Af)--(Bf) -- (Ff)-- (Ef)
%		(Et)--(Ft) -- (Gt)-- (Ht)
%		(Br)--(Cr) -- (Gr)-- (Fr);
%% vetrices
%	\foreach \vertex in {A,...,C} {\node[vertex] at (\vertex) {};}
%	\foreach \vertex in {E,...,H} {\node[vertex] at (\vertex) {};}
%	\node[vertex,fill=gray] at (D) {};       
%}



==> figtex/nfg-informal1-img.tex <==
\begin{tikzpicture}[scale=\s,
		every node/.style={draw, fill=white, node distance=\dist, minimum size=3.5mm, inner sep=0mm},
		every node/.append style={transform shape}
	]
	\node(A) at (0,0) {$=$};
	\draw[]
		(A)--(90:\dist/2.5) (A)--(-90:\dist/2.5);
	\node[draw=none, fill=none, ciliatednode={-90}{3}] at (A) {};
\end{tikzpicture}


==> figtex/planar/planar-imbd2-nfg.tex <==
\begin{tikzpicture}[scale=\s,
		v/.style={\thickness, draw, fill=none, \linetype, \clr, node distance=\dist, minimum size=3mm, inner sep=.2mm},
		d/.style={\thickness, node distance=.5*\dist, draw, \clr, \linetype, minimum width =0mm, minimum height=\dangle, inner sep=0mm},
		%every label/.style={label distance=-5mm},
		every node/.append style={transform shape}
	]
	%\node(r)[v, ciliatednode={90}{2*\minsize}, label=above right:$S_1$] {$=$};
	\node(dumb) at (0,0){};
	\node(r)[v, label={[label distance=-1.5mm, \clr]above right:$S_1$}, above left=2.05cm and 0cm of dumb] {$=$};
	%\node(r)[v, label={[label distance=-1.5mm, \clr]above right:$S_1$}] {$=$};
	\node(y)[v, right of = r, label={[label distance=-1.5mm, \clr]above right:$S_2$}] {$=$};
	\node(ry)[v] at ($(r)!.5!(y)$) {$+$};
	\node(dr1)[d, above of=r, rotate=90]{}; \node(dr2)[d, left of=r]{}; \node(dr3)[d,node
	distance = .8*\dist, below of=r, rotate=90]{};
	\node(dy1)[d, above of=y, rotate=90]{}; \node(dy2)[d, right of=y, rotate=0]{};
	\node(dry)[d, below of=ry, rotate=90, node distance=.3*\dist]{};

	\path[every node/.style={\thickness, \linetype, transform shape},
		every edge/.style={draw, \thickness, \linetype, \clr, transform shape}]
	(r)edge(dr1)edge(dr2)edge(dr3)
	(y)edge(dy1)edge(dy2)
	(ry)edge(y)edge(r) edge(dry);
	\node() at (r)[v, ciliatednode={180}{.5*\minsize}]{};
	\node() at (y)[v, ciliatednode={0}{.5*\minsize}]{};
	\node() at (y)[v, ciliatednode={180}{.5*\minsize}]{};
	\node() at (ry)[v, ciliatednode={0}{.5*\minsize}]{};
	\node() at (ry)[v, ciliatednode={180}{.5*\minsize}]{};
\end{tikzpicture}


==> figtex/planar/planar-imdif1-nfg.tex <==
\begin{tikzpicture}[scale=\s,
		v/.style={draw, fill=white, node distance=\dist, minimum size=3mm, inner sep=.2mm},
		%d/.style={node distance=.4*\dist, minimum size=0mm, inner sep=.1mm},
		d/.style={node distance=.4*\dist, draw, \clr, \linetype, minimum width =0mm, minimum height=\dangle, inner sep=0mm},
		every node/.append style={transform shape}
	]
	\node(a)[v, label=above:$v_1$] {$=$};
	\node(b)[v, right of = a, label=above:$v_2$] {$=$};
	\node(d)[v, below of = a, label=below:$v_5$] {$=$};
	\node(c)[v, below of = b, label=below:$v_4$] {$=$};
	\node(e)[v, right of = b, label=above:$v_3$] {$=$};


	\path[every node/.style={transform shape}]
	(a)edge(b)edge(d)
	(b)edge(c)edge(e)
	(c)edge(d)edge(e)
	;

	\node(ad)[v, ciliatednode={-90}{.5*\minsize}] at ($(a)!.5!(d)$){$+$};
	\node(ab)[v, ciliatednode={0}{.5*\minsize}] at ($(a)!.5!(b)$){$+$};
	\node(bc)[v, ciliatednode={-90}{.5*\minsize}] at ($(b)!.5!(c)$){$+$};
	\node(be)[v, ciliatednode={0}{.5*\minsize}] at ($(b)!.5!(e)$){$+$};
	\node(cd)[v, ciliatednode={180}{.5*\minsize}] at ($(c)!.5!(d)$){$+$};
	\node(ce)[v, ciliatednode={45}{.5*\minsize}] at ($(c)!.5!(e)$){$+$};
	\node(dab)[d, above of=ab,label={[label distance=0mm]below left:$x_{12}$}, rotate=90]{};
\node(dad)[d, left of=ad, label={[xshift=1mm, yshift=0mm]$x_{15}$}]{};
	\node(dbc)[d, left of=bc,label={[label distance=-1mm]below:$x_{24}$}]{};
	\node(dbe)[d, above of=be, label={[label distance=0mm]below left:$x_{23}$},rotate=90]{};
\node(dcd)[d, node distance=.2*\dist, below of=cd, label={[xshift=-2.5mm, yshift=-3mm]$x_{45}$}, rotate=90]{};
\node(dce)[d, right of=ce, label={[xshift=1mm, yshift=0mm]$x_{43}$}]{};

	\path[every node/.style={transform shape}]
	(ab)edge(dab)
	(ad)edge(dad)
	(bc)edge(dbc)
	(be)edge(dbe)
	(ce)edge(dce)
	(cd)edge(dcd)
	;
\end{tikzpicture}


==> figtex/planar/planar-kerbd1-nfg.tex <==
\begin{tikzpicture}[scale=\s,
		v/.style={draw, fill=white, node distance=\dist, minimum size=3mm, inner sep=.2mm},
		vv/.style={draw, fill=none, node distance=\dist, minimum size=3mm, inner sep=.2mm},
		%d/.style={node distance=.4*\dist, minimum size=0mm, inner sep=.1mm},
		d/.style={node distance=.4*\dist, draw, \clr, \linetype, minimum width =0mm, minimum height=\dangle, inner sep=0mm},
		every node/.append style={transform shape}
	]
	\node(a)[v, label=above:$v_1$] {$+$};
	\node(b)[v, right of = a, label=above:$v_2$] {$+$};
	\node(d)[v, below of = a, label=below:$v_5$] {$+$};
	\node(c)[v, below of = b, label=below:$v_4$] {$+$};
	\node(e)[v, right of = b, label=above:$v_3$] {$+$};

	\path[every node/.style={transform shape}]
	(a)edge node(ab)[v]{$=$}(b)edge node(ad)[v]{$=$}(d)
	(b)edge node(bc)[v]{$=$}(c)edge node(be)[v]{$=$}(e)
	(c)edge node(cd)[v]{$=$}(d)edge node(ce)[v]{$=$}(e)
	;
	%\node [label={[xshift=1.0cm, yshift=0.3cm]Label}] {Node};
\node(dab)[d, above of=ab,label={[label distance=0mm]below left:$x_{12}$}, rotate=90]{};
\node(dad)[d, left of=ad, label={[xshift=1mm, yshift=.0mm]$x_{15}$}]{};
\node(dbc)[d, left of=bc,label={[label distance=-1mm]below:$x_{24}$}]{};
\node(dbe)[d, above of=be, label={[label distance=0mm]below left:$x_{23}$},rotate=90]{};
\node(dcd)[d, node distance=.2*\dist, below of=cd, label={[xshift=-2.5mm, yshift=-3mm]$x_{45}$}, rotate=90]{};
\node(dce)[d, right of=ce, label={[xshift=1mm, yshift=0mm]$x_{43}$}]{};
	%\node(dab)[d, above of=ab,label={[label distance=0mm]below left:$x_{st}$}, rotate=90]{};
	%\node(dad)[d, left of=ad]{};
	%\node(dbc)[d, left of=bc,label={[label distance=-1mm]below:$x_{tv}$}]{};
	%\node(dbe)[d, above of=be, label={[label distance=0mm]below left:$x_{tu}$},rotate=90]{};
	%\node(dcd)[d, node distance=.2*\dist, below of=cd, rotate=90]{};
	%\node(dce)[d, right of=ce]{};

	\path[every node/.style={transform shape}]
	(ab)edge(dab)
	(ad)edge(dad)
	(bc)edge(dbc)
	(be)edge(dbe)
	(ce)edge(dce)
	(cd)edge(dcd)
	;
	\node()at(a)[vv, ciliatednode={0}{.5*\minsize}]{}; \node()at(a)[vv, ciliatednode={-90}{.5*\minsize}]{};
	\node()at(b)[vv, ciliatednode={0}{.5*\minsize}]{}; \node()at(b)[vv, ciliatednode={-90}{.5*\minsize}]{};
	\node()at(c)[vv, ciliatednode={180}{.5*\minsize}]{}; \node()at(c)[vv, ciliatednode={45}{.5*\minsize}]{};
\end{tikzpicture}


==> figtex/planar/planar-kerdif2-nfg.tex <==
\begin{tikzpicture}[scale=\s,
	v/.style={\thickness, draw, fill=none, \linetype, \clr, node distance=\dist, minimum size=3mm, inner sep=.2mm},
	d/.style={\thickness, node distance=.5*\dist, draw, \clr, \linetype, minimum width =0mm, minimum height=\dangle, inner sep=0mm},
	%every label/.style={label distance=-5mm},
	every node/.append style={transform shape}
	]
	\node(dumb) at (0,0){};
	\node(r)[v, label={[label distance=-1.5mm, \clr]above right:$S_1$}, above left=2.05cm and 0cm of dumb] {$+$};
	%\node(r)[v, label={[label distance=-1.5mm, \clr]above right:$S_1$}] {$+$};
	\node(y)[v, right of = r, label={[label distance=-1.5mm, \clr]above right:$S_2$}] {$+$};
	\node(ry)[v] at ($(r)!.5!(y)$) {$=$};
	\node(dr1)[d, above of=r, rotate=90]{}; \node(dr2)[d, left of=r]{}; \node(dr3)[d,node
	distance = .8*\dist, below of=r, rotate=90]{};
	\node(dy1)[d, above of=y, rotate=90]{}; \node(dy2)[d, right of=y, rotate=0]{};
	\node(dry)[d, below of=ry, rotate=90, node distance=.3*\dist]{};

	\path[every node/.style={\linetype, transform shape}, every edge/.style={\thickness, draw, \clr, \linetype, transform shape}
	]
	(r)edge(dr1)edge(dr2)edge(dr3)
	(y)edge(dy1)edge(dy2)
	(ry)edge (y)edge(r) edge(dry);
	\node()at(r)[v, ciliatednode={180}{.5*\minsize}]{};
	\node()at(y)[v, ciliatednode={0}{.5*\minsize}]{};
	\node()at(y)[v, ciliatednode={180}{.5*\minsize}]{};
\end{tikzpicture}


==> figtex/square/square-1complex/alternative-version/square-img-bd1.tex <==
\begin{tikzpicture}[
		d/.style={node distance=\c cm, minimum width=0mm, minimum height=\dongle cm},
		every node/.style={node distance=\dist/2, draw, \linetype, fill=white, minimum size=3.0mm,
		inner sep=0mm, transform shape},
		]
% torus grid
	\foreach \x in {0,...,\L}{
		\draw (0,\dist*\x)--(\dist*\L,\dist*\x);
		\draw (\dist*\x, 0)--(\dist*\x, \dist*\L);
	}
% end of grid
	\pgfmathtruncatemacro{\Lminus}{\L-1};
	\foreach \x in {0,...,\L}{
		\foreach \y in {0,...,\L}{
			\node(v\x\y) at (\dist*\x,\dist*\y){$+$};
			\node(dv)[d, above right of=v\x\y, rotate=45]{};
			\draw[\linetype] (v\x\y)--(dv);
		}
	}
	\foreach \x in {0,...,\Lminus}{
		\foreach \y in {1,...,\L}{
			\node(er\x\y)[right of=v\x\y] {$=$};
			\node(eb\x\y)[below of =v\x\y]{$=$};
			%\node(db)[d, right of=eb\x\y]{};
			%\node(dr)[d, above of=er\x\y, rotate=90]{};
			%\draw[\linetype] (er\x\y) -- (dr)   (eb\x\y) -- (db);
		}
	}
	\foreach \x [count=\y] in {0,...,\Lminus}{
		\node(er\x0)[right of=v\x0] {$=$};
		%\node(dr)[d, above of=er\x0, rotate=90]{};
		\node(eb\L\y)[below of=v\L\y] {$=$};
		%\node(db)[d, right of=eb\L\y]{};
		%\draw[\linetype] (er\x0) -- (dr)   (eb\L\y) -- (db);
	}
% ciliation
	\foreach \x in {1,...,\L}{
		\foreach \y in {0,...,\Lminus}{
			\node[draw=none, fill=none, ciliatednode={180}{3}] at (v\x\y){\phantom{$+$}};
			\node[draw=none, fill=none, ciliatednode={90}{3}] at (v\x\y){\phantom{$+$}};
		}
	}
	\foreach \x [count=\y] in {0,...,\Lminus}{
		\node[draw=none, fill=none, ciliatednode={90}{3}] at (v0\x){\phantom{$+$}};
		\node[draw=none, fill=none, ciliatednode={180}{3}] at (v\y\L){\phantom{$+$}};
	}
\end{tikzpicture}


==> figtex/square/square-1complex/alternative-version/square-nfga-part.tex <==
\begin{tikzpicture}[
		>=latex,
		d/.style={node distance=\c cm, draw=none, minimum width=0mm, minimum height=\dongle cm},
		every node/.style={node distance=\dist/2, draw, \linetype, fill=white, minimum size=3.0mm,
		inner sep=0mm, transform shape},
		every path/.style={\clr, \linetype},
		]
	\def\L{1}
% torus grid
	\foreach \x in {0,...,\L}{
		\draw (0,\dist*\x)--(\dist*\L,\dist*\x);
		\draw (\dist*\x, 0)--(\dist*\x, \dist*\L);
	}
% end of grid
	\pgfmathtruncatemacro{\Lminus}{\L-1};
	\foreach \x in {0,...,\L}{
		\foreach \y in {0,...,\L}{
			\node(v\x\y) at (\dist*\x,\dist*\y){$+$};
			\node(dv)[d, below left of=v\x\y, rotate=45]{};
			\draw[\linetype, ->] (v\x\y)--(dv);
		}
	}
	\foreach \x in {0,...,\Lminus}{
		\foreach \y in {1,...,\L}{
			\node(er\x\y)[right of=v\x\y] {$=$};
			\node(eb\x\y)[below of =v\x\y]{$=$};
			\node(db)[d, right of=eb\x\y]{};
			\node(dr)[d, above of=er\x\y, rotate=90]{};
			\draw[\linetype, <-] (er\x\y) -- (dr);
			\draw[\linetype, <-](eb\x\y) -- (db);
		}
	}
	\foreach \x [count=\y] in {0,...,\Lminus}{
		\node(er\x0)[right of=v\x0] {$=$};
		\node(dr)[d, above of=er\x0, rotate=90]{};
		\node(eb\L\y)[below of=v\L\y] {$=$};
		\node(db)[d, left of=eb\L\y]{};
		\draw[\linetype, <-] (er\x0) -- (dr);
		\draw[\linetype, <-] (eb\L\y) -- (db);
	}
% ciliation
	\foreach \x in {0,...,\Lminus}{
		\foreach \y in {1,...,\L}{
			\node[draw=none, fill=none, ciliatednode={0}{3}] at (v\x\y){\phantom{$+$}};
			\node[draw=none, fill=none, ciliatednode={-90}{3}] at (v\x\y){\phantom{$+$}};
		}
	}
	\foreach \x [count=\y] in {0,...,\Lminus}{
		\node[draw=none, fill=none, ciliatednode={0}{3}] at (v\x0){\phantom{$+$}};
		\node[draw=none, fill=none, ciliatednode={-90}{3}] at (v\L\y){\phantom{$+$}};
	}
\end{tikzpicture}


==> figtex/square/square-1complex/alternative-version/square-nfga.tex <==
\begin{tikzpicture}[
		>=latex,
		d/.style={node distance=\c cm, draw=none, minimum width=0mm, minimum height=\dongle cm},
		every node/.style={node distance=\dist/2, draw, \linetype, fill=white, minimum size=3.0mm,
		inner sep=0mm, transform shape},
		]
% torus grid
	\foreach \x in {0,...,\L}{
		\draw (0,\dist*\x)--(\dist*\L,\dist*\x);
		\draw (\dist*\x, 0)--(\dist*\x, \dist*\L);
	}
% end of grid
	\pgfmathtruncatemacro{\Lminus}{\L-1};
	\foreach \x in {0,...,\L}{
		\foreach \y in {0,...,\L}{
			\node(v\x\y) at (\dist*\x,\dist*\y){$+$};
			\node(dv)[d, above right of=v\x\y, rotate=45]{};
			\draw[\linetype, ->] (v\x\y)--(dv);
		}
	}
	\foreach \x in {0,...,\Lminus}{
		\foreach \y in {1,...,\L}{
			\node(er\x\y)[right of=v\x\y] {$=$};
			\node(eb\x\y)[below of =v\x\y]{$=$};
			\node(db)[d, left of=eb\x\y]{};
			\node(dr)[d, below of=er\x\y, rotate=90]{};
			\draw[\linetype, <-] (er\x\y) -- (dr);
			\draw[\linetype, <-](eb\x\y) -- (db);
		}
	}
	\foreach \x [count=\y] in {0,...,\Lminus}{
		\node(er\x0)[right of=v\x0] {$=$};
		\node(dr)[d, below of=er\x0, rotate=90]{};
		\node(eb\L\y)[below of=v\L\y] {$=$};
		\node(db)[d, left of=eb\L\y]{};
		\draw[\linetype, <-] (er\x0) -- (dr);
		\draw[\linetype, <-] (eb\L\y) -- (db);
	}
% ciliation
	\foreach \x in {0,...,\Lminus}{
		\foreach \y in {1,...,\L}{
			\node[draw=none, fill=none, ciliatednode={0}{3}] at (v\x\y){\phantom{$+$}};
			\node[draw=none, fill=none, ciliatednode={-90}{3}] at (v\x\y){\phantom{$+$}};
		}
	}
	\foreach \x [count=\y] in {0,...,\Lminus}{
		\node[draw=none, fill=none, ciliatednode={0}{3}] at (v\x0){\phantom{$+$}};
		\node[draw=none, fill=none, ciliatednode={-90}{3}] at (v\L\y){\phantom{$+$}};
	}
\end{tikzpicture}


==> figtex/square/square-1complex/alternative-version/square-nfgb-part.tex <==
\begin{tikzpicture}[
		>=latex,
		d/.style={node distance=\c cm, draw=none, minimum width=0mm, minimum height=\dongle cm},
		every node/.style={node distance=\dist/2, draw, \linetype, fill=white, minimum size=3.0mm,
		inner sep=0mm, transform shape},
		every path/.style={\clr, \linetype},
		]
	\def\L{1}
% torus grid
	\foreach \x in {0,...,\L}{
		\draw (0,\dist*\x)--(\dist*\L,\dist*\x);
		\draw (\dist*\x, 0)--(\dist*\x, \dist*\L);
	}
% end of grid
	\pgfmathtruncatemacro{\Lminus}{\L-1};
	\foreach \x in {0,...,\L}{
		\foreach \y in {0,...,\L}{
			\node(v\x\y) at (\dist*\x,\dist*\y){$=$};
			\node(dv)[d, below left of=v\x\y, rotate=45]{};
			\draw[\linetype, <-] (v\x\y)--(dv);
		}
	}
	\foreach \x in {0,...,\Lminus}{
		\foreach \y in {1,...,\L}{
			\node(er\x\y)[right of=v\x\y] {$+$};
			\node(eb\x\y)[below of =v\x\y]{$+$};
			\node(db)[d, right of=eb\x\y]{};
			\node(dr)[d, above of=er\x\y, rotate=90]{};
			\draw[\linetype, ->] (er\x\y) -- (dr);
			\draw[\linetype, ->](eb\x\y) -- (db);
		}
	}
	\foreach \x [count=\y] in {0,...,\Lminus}{
		\node(er\x0)[right of=v\x0] {$+$};
		\node(dr)[d, above of=er\x0, rotate=90]{};
		\node(eb\L\y)[below of=v\L\y] {$+$};
		\node(db)[d, right of=eb\L\y]{};
		\draw[\linetype, ->] (er\x0) -- (dr);
		\draw[\linetype, ->] (eb\L\y) -- (db);
	}
%% ciliation
%	\foreach \x in {0,...,\Lminus}{
%		\foreach \y in {1,...,\L}{
%			\node[draw=none, fill=none, ciliatednode={0}{3}] at (v\x\y){\phantom{$+$}};
%			\node[draw=none, fill=none, ciliatednode={-90}{3}] at (v\x\y){\phantom{$+$}};
%		}
%	}
%	\foreach \x [count=\y] in {0,...,\Lminus}{
%		\node[draw=none, fill=none, ciliatednode={0}{3}] at (v\x0){\phantom{$+$}};
%		\node[draw=none, fill=none, ciliatednode={-90}{3}] at (v\L\y){\phantom{$+$}};
%	}
% ciliation
	\foreach \x in {1,...,\L}{
		\foreach \y in {0,...,\Lminus}{
			\node[draw=none, fill=none, ciliatednode={180}{3}] at (v\x\y){\phantom{$+$}};
			\node[draw=none, fill=none, ciliatednode={90}{3}] at (v\x\y){\phantom{$+$}};
		}
	}
	\foreach \x [count=\y] in {0,...,\Lminus}{
		\node[draw=none, fill=none, ciliatednode={90}{3}] at (v0\x){\phantom{$+$}};
		\node[draw=none, fill=none, ciliatednode={180}{3}] at (v\y\L){\phantom{$+$}};
	}
\end{tikzpicture}


==> figtex/square/square-1complex/alternative-version/square-nfgb.tex <==
\begin{tikzpicture}[
		>=latex,
		d/.style={node distance=\c cm, draw=none, minimum width=0mm, minimum height=\dongle cm},
		every node/.style={node distance=\dist/2, draw, \linetype, fill=white, minimum size=3.0mm,
		inner sep=0mm, transform shape},
		]
% torus grid
	\foreach \x in {0,...,\L}{
		\draw (0,\dist*\x)--(\dist*\L,\dist*\x);
		\draw (\dist*\x, 0)--(\dist*\x, \dist*\L);
	}
% end of grid
	\pgfmathtruncatemacro{\Lminus}{\L-1};
	\foreach \x in {0,...,\L}{
		\foreach \y in {0,...,\L}{
			\node(v\x\y) at (\dist*\x,\dist*\y){$=$};
			\node(dv)[d, above right of=v\x\y, rotate=45]{};
			\draw[\linetype, <-] (v\x\y)--(dv);
		}
	}
	\foreach \x in {0,...,\Lminus}{
		\foreach \y in {1,...,\L}{
			\node(er\x\y)[right of=v\x\y] {$+$};
			\node(eb\x\y)[below of =v\x\y]{$+$};
			\node(db)[d, left of=eb\x\y]{};
			\node(dr)[d, below of=er\x\y, rotate=90]{};
			\draw[\linetype, ->] (er\x\y) -- (dr);
			\draw[\linetype, ->](eb\x\y) -- (db);
		}
	}
	\foreach \x [count=\y] in {0,...,\Lminus}{
		\node(er\x0)[right of=v\x0] {$+$};
		\node(dr)[d, below of=er\x0, rotate=90]{};
		\node(eb\L\y)[below of=v\L\y] {$+$};
		\node(db)[d, left of=eb\L\y]{};
		\draw[\linetype, ->] (er\x0) -- (dr);
		\draw[\linetype, ->] (eb\L\y) -- (db);
	}
%% ciliation
%	\foreach \x in {0,...,\Lminus}{
%		\foreach \y in {1,...,\L}{
%			\node[draw=none, fill=none, ciliatednode={0}{3}] at (v\x\y){\phantom{$+$}};
%			\node[draw=none, fill=none, ciliatednode={-90}{3}] at (v\x\y){\phantom{$+$}};
%		}
%	}
%	\foreach \x [count=\y] in {0,...,\Lminus}{
%		\node[draw=none, fill=none, ciliatednode={0}{3}] at (v\x0){\phantom{$+$}};
%		\node[draw=none, fill=none, ciliatednode={-90}{3}] at (v\L\y){\phantom{$+$}};
%	}
% ciliation
	\foreach \x in {1,...,\L}{
		\foreach \y in {0,...,\Lminus}{
			\node[draw=none, fill=none, ciliatednode={180}{3}] at (v\x\y){\phantom{$+$}};
			\node[draw=none, fill=none, ciliatednode={90}{3}] at (v\x\y){\phantom{$+$}};
		}
	}
	\foreach \x [count=\y] in {0,...,\Lminus}{
		\node[draw=none, fill=none, ciliatednode={90}{3}] at (v0\x){\phantom{$+$}};
		\node[draw=none, fill=none, ciliatednode={180}{3}] at (v\y\L){\phantom{$+$}};
	}
\end{tikzpicture}


==> figtex/torus/cube-imdif1-less.tex <==
\begin{tikzpicture}[scale=\dist] 
	\cubebdthreex{0}{0}{0}{+}{=}{dump}{dump}{none} % 'none' will treat dual faces as primal edges
\end{tikzpicture} 




==> figtex/torus/cube-kerbd1-less.tex <==
\begin{tikzpicture}[scale=\dist] 
	\cubebdthreex{0}{0}{0}{=}{+}{dump}{dump}{none} % 'none' will treat dual faces as primal edges
\end{tikzpicture} 




==> figtex/torus/cube-kerdif2.tex <==
\begin{tikzpicture}[scale=\dist] 
	\def\nx{0}
	\def\ny{0}
	\def\nz{0}
	\foreach \x in {0,...,\nx}
	\foreach \x in {0,...,\nx}
		\foreach \y in {0,...,\ny}
			\foreach \z in {\nz,...,0}
				{
					\cubebdtwo{\x}{\y}{\z}{+}{=}{none}{half}{none}
				}
\end{tikzpicture} 


==> figtex/torus/preamble.tex <==

\usepackage{balance}
\usepackage[export]{adjustbox}



\usepackage{tikz}
\usetikzlibrary{calc, arrows, decorations.markings, shapes, positioning, 3d}
\usepackage{xifthen}
% calc for node between two nodes
% decoration for ciliation

\usepackage{calc} % Included for the clockwise arrow
\usepackage{subfigure}
\usepackage{caption}
\usepackage{graphicx}
\usepackage{comment}
\usepackage{color}






==> figtex/torus/tikz-preamble.tex <==
\input{/home/alio//Dropbox/kwextended2/cube} % \angle is defined here
\def\extend{.4}
\def\extendclr{gray!50}
\def\extendclr{red!50}
\input{/home/alio//Dropbox/kwextended2/cube-orient-ext}
%\input{cube-orient}
%\input{cubenfg3}

%\input{cubenfgbd3ext}
\input{/home/alio//Dropbox/kwextended2/cubenfgbd3}
\input{/home/alio//Dropbox/kwextended2/cubenfgbd2}
%\input{cubenfgbd1ext}
\input{/home/alio//Dropbox/kwextended2/cubenfgbd1}
%\input{cubenfgbd2_2}
%\input{cubenfg}
\input{/home/alio//Dropbox/kwextended2/cubedang}

\input{/home/alio//Dropbox/kwextended2/vstyles-common}



% Face orientation 


%\begin{tikzpicture}
%\begin{scope}[canvas is xy plane at z=2]
%%\draw (0,0) circle (1cm);
%%\draw (-1,0) -- (1,0) (0,-1) -- (0,1);
%%\counterclockwise{$S_3$}
%\draw (0,1.0) arc (85:-240:1.0);%
%\end{scope}
%\end{tikzpicture}

\makeatletter
\newlength\@SizeOfCirc%
\newcommand{\CricArrowRight}[1]{%
	\setlength{\@SizeOfCirc}{\maxof{\widthof{#1}}{\heightof{#1}}}%
	\tikz [>=angle 90, x=1.0ex,y=1.0ex,line width=.1ex, draw=black]%
	\draw [->,anchor=center]%
		node[fill=none, draw=none] (0,0) {#1}%
		(0,1.0\@SizeOfCirc) arc (85:-240:1.0\@SizeOfCirc);%
}%
\newcommand{\clockwise}[1]{%
	\setlength{\@SizeOfCirc}{\maxof{\widthof{#1}}{\heightof{#1}}}%
	\tikz [>=angle 90, x=1.0ex,y=1.0ex,line width=.1ex, draw=black]%
	\draw [->,anchor=center]%
		node[fill=none, draw=none] (0,0) {#1}%
		(0,1.0\@SizeOfCirc) arc (85:-240:1.0\@SizeOfCirc);%
}%
\newcommand{\counterclockwise}[1]{%
	\setlength{\@SizeOfCirc}{\maxof{\widthof{#1}}{\heightof{#1}}}%
	\begin{tikzpicture}[>=angle 90, x=1.0ex,y=1.0ex,line width=.1ex, draw=black]%
	\draw [->,anchor=center]%
		node[fill=none, draw=none] (0,0) {#1}%
		(0,1.0\@SizeOfCirc) arc (-275:40:1.0\@SizeOfCirc);%
	\end{tikzpicture}
}%
%
\makeatother


\def\clocksize{4}
\def\angstart{0}
\def\angend{45}
\newcommand{\clockxy}[1]{%
	\tikz[>=angle 90, x=1.0ex,y=1.0ex,line width=.1ex, draw=black]%
	\draw [->,anchor=center]%
		node[fill=none, draw=none] (0,0) {#1}%
		(0,{1*\clocksize}) arc (0:\angend-360:{.75*\clocksize});%
}%
\newcommand{\clockxz}[1]{%
	\tikz[>=angle 90, x=1.0ex,y=1.0ex,line width=.1ex, draw=black]%
	\draw [->,anchor=center]%
		node[fill=none, draw=none] (0,0) {#1}%
		(0,{.5*\clocksize}) arc (0:\angend-360:{\clocksize*\cosine} and {\clocksize*\sine});%
}%
\newcommand{\clockyz}[1]{%
	\tikz[>=angle 90, x=1.0ex,y=1.0ex,line width=.1ex, draw=black]%
	\draw [->,anchor=center]%
		node[fill=none, draw=none] (0,0) {#1}%
		(0,{.5*\clocksize}) arc (0:\angend-360:{\clocksize*\cosine} and {\clocksize*\sine});%
}%
%
\newcommand{\counterclockxy}[1]{%
	\tikz[>=angle 90, x=1.0ex,y=1.0ex,line width=.1ex, draw=black]%
	\draw [->,anchor=center]%
		node[fill=none, draw=none] (0,0) {#1}%
		(0,{1*\clocksize}) arc (0:\angend-360:{.75*\clocksize});%
}%
\newcommand{\counterclockxz}[1]{%
	\tikz[>=angle 90, x=1.0ex,y=1.0ex,line width=.1ex, draw=black]%
	\draw [->,anchor=center]%
		node[fill=none, draw=none] (0,0) {#1}%
		(0,{.5*\clocksize}) arc (-275:40:{\clocksize*\cosine} and {\clocksize*\sine});%
}%
\newcommand{\counterclockyz}[1]{%
	\tikz[>=angle 90, x=1.0ex,y=1.0ex,line width=.1ex, draw=black]%
	\draw [->,anchor=center]%
		node[fill=none, draw=none] (0,0) {#1}%
		(0,{.5*\clocksize}) arc (-270:40:{\clocksize*\cosine} and {\clocksize*\sine});%
}%
%


%\newcommand{\clockxz}[1]{%
%	\settowidth{\SizeofCirc}{\pgfinterruptpicture A \endpgfinterruppicture}%
%	\begin{tikzpicture}[>=angle 90, x=1.0ex,y=1.0ex,line width=.1ex, draw=black]%
%%\begin{scope}[canvas is xz plane at y=0]
%	\draw [->,anchor=center]%
%		node[fill=none, draw=none] (0,0) {#1}%
%		%(0,1.0\@SizeOfCirc) arc (85:-240:1\@SizeOfCirc);%
%		(0,1.0\SizeofCirc) arc (85:-240:1.0\SizeofCirc);%
%%\end{scope}
%	\end{tikzpicture}
%}%

% Ciliation take 2
\tikzstyle ciliation=[circle,draw,fill=white,inner sep=0pt, minimum size=#1]
\tikzset{ ciliatednode/.style 2 args
	={ pin={[pin distance=0mm, ciliation=#2]#1:{}} }
	%={pin={} }
}
% gray ciliation
\tikzstyle gciliation=[gray, circle,draw,fill=white,inner sep=0pt, minimum size=#1]
\tikzset{ gciliatednode/.style 2 args
	={ pin={[pin distance=0mm, gciliation=#2]#1:{}} }
	%={pin={} }
}
% extend ciliation
\tikzstyle extendciliation=[\extendclr, circle,draw,fill=white,inner sep=0pt, minimum size=#1]
\tikzset{ extendciliatednode/.style 2 args
	={ pin={[pin distance=0mm, extendciliation=#2]#1:{}} }
	%={pin={} }
}

% dongle
\tikzset{ --|/.style={
  decoration={ markings,
  mark=at position 1 with {\pgftransformscale{1.5}\arrowreversed[line width=0mm]{|}}},
  postaction={decorate}
  }
}


%%\newcommand\cube{
%\newcommand\cube[3]{
%%\fill[fill=red!40, draw=black,shift={(0:#1)},shift={(90:#2)}, shift={(45:#3)}]
%% define the points  
%	\def\angle{30}
%	\pgfmathsetmacro\cos{cos(\angle)}
%	\pgfmathsetmacro\sin{sin(\angle)}
%	\path[shift={(0:#1)},shift={(90:#2)}, shift={(\angle:#3*\cos)}]
%		%(0,0)     coordinate (A)  (1,0)     coordinate (B) % bottom
%		%(1.5,0.5) coordinate (C)  (0.5,0.5) coordinate (D)
%		%(0,1)     coordinate (E)  (1,1)     coordinate (F) % top  add 1 for y
%		%(1.5,1.5) coordinate (G)  (0.5,1.5) coordinate (H);
%		(0,0)  coordinate (A)  (1,0)     coordinate (B) % bottom
%		+(\angle:\cos) coordinate (C)  (\angle:\cos) coordinate (D)
%		(0,1)  coordinate (E) +(\angle:\cos) coordinate (H)   % top  add 1 for y
%		(1,1)  coordinate (F) +(\angle:\cos) coordinate (G)  ;
%%        ($(A)!0.5!(C)$) coordinate (O)   % middle of A--C
%%        ($(E)!0.5!(G)$) coordinate (P);%   
%	\draw[draw=black]
%		(A) -- (E) (B) -- (F) (C) -- (G)  % lateral 
%		(A) -- (B) -- (C) % bottom 
%		(E) -- (F) -- (G) -- (H) -- (E); % top
%	% dashed is an option
%	\draw[fill=red!40, draw=black]
%		(D) -- (H) (D) -- (C) (D) -- (A);  
%% shading
%	%\node[fill=white,opacity=.8, minimum height=1.47cm, minimum width=1.47cm] at ($(A)+(.5,.5)$) {};
%		\def\gap{.99}
%		% front
%		\node[inner sep=0,minimum size=0](cf) at (barycentric cs:A=1,B=1,F=1,E=1){};
%		\path(cf) -- coordinate[pos=\gap] (Af) (A.0);
%		\path(cf) -- coordinate[pos=\gap] (Bf) (B);
%		\path(cf) -- coordinate[pos=\gap] (Ff) (F);
%		\path(cf) -- coordinate[pos=\gap] (Ef) (E);
%		\draw(F)--(Ff);
%		% right
%		\node[inner sep=0,minimum size=0](cr) at (barycentric cs:B=1,C=1,G=1,F=1){};
%		\path(cr) -- coordinate[pos=\gap] (Br) (B);
%		\path(cr) -- coordinate[pos=\gap] (Cr) (C);
%		\path(cr) -- coordinate[pos=\gap] (Gr) (G);
%		\path(cr) -- coordinate[pos=\gap] (Fr) (F);
%		% top
%		\node[inner sep=0,minimum size=0](ct) at (barycentric cs:E=1,F=1,G=1,H=1){};
%		\path(ct) -- coordinate[pos=\gap] (Et) (E);
%		\path(ct) -- coordinate[pos=\gap] (Gt) (G);
%		\path(ct) -- coordinate[pos=\gap] (Ft) (F);
%		\path(ct) -- coordinate[pos=\gap] (Ht) (H);
%
%	\path[fill=white,fill opacity=.6]
%		(Af)--(Bf) -- (Ff)-- (Ef)
%		(Et)--(Ft) -- (Gt)-- (Ht)
%		(Br)--(Cr) -- (Gr)-- (Fr);
%% vetrices
%	\foreach \vertex in {A,...,C} {\node[vertex] at (\vertex) {};}
%	\foreach \vertex in {E,...,H} {\node[vertex] at (\vertex) {};}
%	\node[vertex,fill=gray] at (D) {};       
%}



==> tikzexternalize.tex <==
\usepackage{pgfplots}
\usetikzlibrary{external}
\tikzexternalize[prefix=tikzpdf/]
\expandafter\gdef\csname c@tikzext@no@\pgfkeysvalueof{/tikz/external/figure name}\endcsname{1}%

